Improving RNN-Transducers with Acoustic LookAhead

RNN-Transducers (RNN-Ts) have gained widespread acceptance as an end-to-end model for speech to text conversion because of their high accuracy and streaming capabilities. A typical RNN-T independently encodes the input audio and the text context, and combines the two encodings by a thin joint network. While this architecture provides SOTA streaming accuracy, it also makes the model vulnerable to strong LM biasing which manifests as multi-step hallucination of text without acoustic evidence. In this paper we propose LookAhead that makes text representations more acoustically grounded by looking ahead into the future within the audio input. This technique yields a significant 5%-20% relative reduction in word error rate on both in-domain and out-of-domain evaluation sets.

==> ablation_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|cccc|}
\hline
Base Model              & LookAhead type       & dev-clean & test-clean & dev-other & test-other \\ \hline
\multirow{4}{*}{Small}  & Baseline             & 11.5      & 11.7       & 29.3      & 29.9       \\
                        & Greedy AcousticFrame & 10.2      & 10.4       & 26.8      & 27.6       \\
                        & Conv                 & 9.6       & 10.0       & 26.8      & 27.6       \\
                        & Greedy Argmax        & \textbf{9.4}       & \textbf{9.7}        & \textbf{25.4}      & \textbf{26.0}       \\ \hline
\multirow{4}{*}{Medium} & Baseline             & 7.1       & 7.6        & 20.5      & 20.8       \\
                        & Greedy AcousticFrame & 9.5         & 9.9          & 25.3         & 26.2          \\
                        & Conv                 & 9.6       & 10.2       & 25.5      & 26.3       \\
                        & Greedy Argmax        & \textbf{6.4}       & \textbf{6.6}        & \textbf{18.8}      & \textbf{19.1}       \\ \hline
\end{tabular}%
}
\caption{Experiments to determine best type of \sysname}
\label{tab:ablations_la_type}
\end{table*}

==> laToken_ablation.tex <==
\begin{table*}
\begin{tabular}{|l|c|c|c|c|}
\hline
Model & dev\textsubscript{clean} & test\textsubscript{clean} & dev\textsubscript{other} & test\textsubscript{other}\\
\hline
Baseline & 7.1 & 7.6 & 20.5 & 20.8\\
$\sysname \Delta w$=2 & 6.5 & 6.9 & 18.8 & 19.0\\
$\sysname \Delta w=3$ & 6.4 & 6.6 & 18.8 & 19.1\\
$\sysname \Delta w=5$ & 6.4 & 6.8 & 18.9 & 18.9\\
\hline
\end{tabular}
\caption{Effect of number of future tokens on \sysname}
%\label{tab:la_ablation}
\end{table*}


==> rare_word_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!]
\setlength\tabcolsep{3.0pt}
\resizebox{\textwidth}{!}{%}
\begin{tabular}{|l|cllllllcllllllclclllccllclll|}
\hline
\multirow{2}{*}{Model} & \multicolumn{28}{c|}{Libri-test}                                                                                                                                                                                                                                  \\ \cline{2-29} 
                       & \multicolumn{7}{c}{dev-clean}                                  & \multicolumn{7}{c}{test-clean}                                 & \multicolumn{7}{c}{dev-other}                                  & \multicolumn{7}{c|}{test-other}                                \\ \hline
Baseline               & \multicolumn{7}{c}{\textbf{20.00}}                             & \multicolumn{7}{c}{21.77}                                      & \multicolumn{7}{c}{48.35}                                      & \multicolumn{7}{c|}{51.67}                                     \\
\sysname               & \multicolumn{7}{c}{20.33}                                      & \multicolumn{7}{c}{\textbf{20.05}}                             & \multicolumn{7}{c}{\textbf{47.16}}                             & \multicolumn{7}{c|}{\textbf{50.69}}                            \\ \hline
\multirow{2}{*}{Model} & \multicolumn{28}{c|}{MCV-test}                                                                                                                                                                                                                                    \\ \cline{2-29} 
                       & \multicolumn{4}{c}{US}             & \multicolumn{4}{l}{Eng}            & \multicolumn{4}{l}{Can}            & \multicolumn{4}{l}{Ind}            & \multicolumn{4}{c}{Scot}           & \multicolumn{4}{c}{Phil}           & \multicolumn{4}{c|}{HK}             \\ \cline{2-29} 
Baseline               & \multicolumn{4}{c}{61.14}          & \multicolumn{4}{l}{63.36}          & \multicolumn{4}{l}{46.17}          & \multicolumn{4}{l}{85.24}          & \multicolumn{4}{c}{60.69}          & \multicolumn{4}{c}{61.22}          & \multicolumn{4}{c|}{70.73}          \\
\sysname               & \multicolumn{4}{c}{\textbf{58.72}} & \multicolumn{4}{l}{\textbf{59.88}} & \multicolumn{4}{l}{\textbf{41.50}} & \multicolumn{4}{l}{\textbf{84.41}} & \multicolumn{4}{c}{\textbf{57.99}} & \multicolumn{4}{c}{\textbf{58.26}} & \multicolumn{4}{c|}{\textbf{67.71}} \\ \hline
\end{tabular}%
}
\caption{Rare-WER comparison of baseline vs \sysname on \textsc{L100+P}.}
\label{tab:rare_table_long}

\end{table*}

==> rare_word_table_dont_use.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\setlength\tabcolsep{3.0pt}
\resizebox{\textwidth}{!}{%}
\begin{tabular}{|l|l|cccc|ccccccc|}
\hline
\multirow{2}{*}{Word-type}   & \multirow{2}{*}{Model} & \multicolumn{4}{c|}{Libri-Test}                   & \multicolumn{7}{c|}{MCV-Test}                                                            \\ \cline{3-13} 
                             &                        & dev-clean  & test-clean & dev-other  & test-other & US         & Eng        & Can        & Ind        & Scot       & Phil       & HK         \\ \hline
\multirow{2}{*}{Rare Word}   & Baseline               & 20.00/0.19 & 21.77/0.21 & 48.35/0.28 & 51.67/0.48 & 61.14/0.79 & 63.36/1.13 & 46.17/0.91 & 85.24/0.74 & 60.69/0.82 & 61.22/0.69 & 70.73/0.96 \\
                             & \sysname               & 20.33/0.25 & 20.05/0.21 & 47.16/0.27 & 50.69/0.47 & 58.72/0.77 & 59.88/1.11 & 41.50/0.88 & 84.41/0.74 & 57.99/0.88 & 58.26/0.69 & 67.71/0.92 \\ \hline
\multirow{2}{*}{Unseen Word} & Baseline               & 53.45/0.76 & 51.14/0.64 & 44.25/0.99 & 48.63/0.81 & 46.54/1.59 & 58.17/2.04 & 58.04/1.57 & 44.53/1.56 & 57.51/1.60 & 52.07/1.53 & 50.07/1.71 \\
                             & \sysname               & 55.08/0.72 & 52.38/0.65 & 45.71/0.96 & 50.97/0.80 & 45.88/1.59 & 57.00/2.02 & 57.98/1.54 & 43.55/1.56 & 57.97/1.60 & 52.92/1.52 & 50.10/1.72 \\ \hline
\end{tabular}%
}
\caption{Rare and unseen word analysis baseline vs \sysname on \textsc{L100+P}. The numbers presented are \%\emph{WER}}
\label{tab:rare_table}
\end{table*}

==> table_5000to500.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cccc|cccccccl|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Model}} & \multicolumn{4}{c|}{Librispeech-Test}                                                                          & \multicolumn{8}{c|}{MCV-Test}                                                                                                                                                                           \\ \cline{2-13} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{dev-clean} & \multicolumn{1}{c|}{test-clean} & \multicolumn{1}{c|}{dev-other} & test-other & \multicolumn{1}{c|}{US}   & \multicolumn{1}{c|}{Eng}  & \multicolumn{1}{c|}{Can}  & \multicolumn{1}{c|}{Ind}  & \multicolumn{1}{c|}{Scot} & \multicolumn{1}{c|}{Phil} & \multicolumn{1}{c|}{HK}   & Avg \\ \hline
Baseline                                     & \multicolumn{1}{c|}{4.2}       & \multicolumn{1}{c|}{4.5}        & \multicolumn{1}{c|}{13.5}      & 13.1       & \multicolumn{1}{c|}{38.1} & \multicolumn{1}{c|}{19.5} & \multicolumn{1}{c|}{23.6} & \multicolumn{1}{c|}{56.9} & \multicolumn{1}{c|}{30.2} & \multicolumn{1}{c|}{34.4} & \multicolumn{1}{c|}{39.1} &     \\ \hline
\sysname                                     & \multicolumn{1}{c|}{\textbf{4.0}}       & \multicolumn{1}{c|}{\textbf{4.3}}        & \multicolumn{1}{c|}{\textbf{12.8}}      & \textbf{12.5}       & \multicolumn{1}{c|}{\textbf{36.9}} & \multicolumn{1}{c|}{\textbf{19.2}} & \multicolumn{1}{c|}{\textbf{22.5}} & \multicolumn{1}{c|}{\textbf{56.6}} & \multicolumn{1}{c|}{\textbf{28.9}} & \multicolumn{1}{c|}{\textbf{33.2}} & \multicolumn{1}{c|}{\textbf{37.5}} &     \\ \hline
\end{tabular}}
\caption{Comparison of \sysname with Baseline with vocabulary of $500$ on a converged baseline of vocabulary of size $5000$.}
\label{tab:libri_500Vocab}
\end{table*}
